Robust Semi-Supervised Monocular Depth Estimation with Reprojected Distances

Dense depth estimation from a single image is a key problem in computer vision, with exciting applications in a multitude of robotic tasks. Initially viewed as a direct regression problem, requiring annotated labels as supervision at training time, in the past few years a substantial amount of work has been done in self-supervised depth training based on strong geometric cues, both from stereo cameras and more recently from monocular video sequences. In this paper we investigate how these two approaches (supervised & self-supervised) can be effectively combined, so that a depth model can learn to encode true scale from sparse supervision while achieving high fidelity local accuracy by leveraging geometric cues. To this end, we propose a novel supervised loss term that complements the widely used photometric loss, and show how it can be used to train robust semi-supervised monocular depth estimation models. Furthermore, we evaluate how much supervision is actually necessary to train accurate scale-aware monocular depth models, showing that with our proposed framework, very sparse LiDAR information, with as few as 4 beams (less than 100 valid depth values per image), is enough to achieve results competitive with the current state-of-the-art.

==> sections/06supmat.tex <==
% \section{More comparison to state-of-the-arts under different settings}

% \section{Extensive analysis on loss weights}

% Since self-supervised loss and supervised loss work jointly in the weakly supervised setting, it is expected that different loss weights will lead to different model performance. To better analysis our proposed model and better understand the weakly supervised monocular depth estimation, we conduct further analysis along the 2 axis in the following sections.
%\subsection{sensitivity to loss weights of supervised losses}

\section{Self-Supervised and Supervised Losses Trade-Off}

Our proposed semi-supervised loss (Eq. 1, main text) is composed of three individual terms: $\mathcal{L}_{photo}$, representing the self-supervised photometric loss, $\mathcal{L}_{smooth}$, representing a self-supervised smoothness depth regularizer, and $\mathcal{L}_{rep}$, representing the proposed supervised reprojected distance loss. Determining the correct balance between these terms is an important part of the training protocol, and in this section we discuss the effects that $\lambda_{rep}$, or the ratio between the self-supervised and supervised components of the loss, has in our overall results.

Interestingly, we did not notice any meaningful changes in numerical results when $\lambda_{rep}$ varies, even if this variation is by a few orders of magnitude. However, there was a significant difference in how the resulting depth maps are visually represented, as depicted in Fig. \ref{fig:change_lambda}. In particular, larger values for $\lambda_{rep}$ promote a worse reconstruction of areas not observed by the LiDAR sensor. We suspect that this behavior is due to the supervised term of the loss overwhelming the self-supervised terms, which hinders the learning of denser, smoother depth maps via the photometric loss. This is supported by the fact that this is a typical behavior of purely supervised depth learning algorithms, where the loss is never calculated in areas where there are no valid depth values. When further lowering $\lambda_{rep}$, we started to see degradation in numerical results, indicating that the photometric loss was being over-represented in the loss and scale was not being learned properly, which led us to elect $\lambda_{rep}=10^4$ as the optimal value for our proposed semi-supervised loss. 



\input{sections/06supmat_tradeoff.tex}

\section{Degradation in the Number of Supervised Frames}
In this section, we provide analysis of our model robustness to another type of degradation in supervision: the number of depth labels available. This is particularly useful as a way to combine large unlabeled datasets, produced without any sort of supervision, with a small amount of labeled images, obtained separately under more controlled circumstances. Our training schedule, on the KITTI dataset, consists of producing two separate splits:
\begin{itemize}
\item \textbf{Unlabeled ($\mathcal{U}$)}: All available images (39810, following the pre-processing steps of \cite{zhou2017unsupervised}) are maintained, discarding all depth information.
\item \textbf{Supervised ($\mathcal{S}$)}: $N$ images are randomly selected from the entire dataset and maintained, alongside their corresponding \textit{Annotated} depth information.
\end{itemize}

Afterwards, training is performed as instructed, however at each step half the batch size is sampled from $\mathcal{U}$ and half from $\mathcal{S}$, with the former not contributing for the proposed reprojected distance loss $\mathcal{L}_{rep}$ during loss calculation. Note that $\mathcal{S}$ is sampled with replacement, so the same labeled images can be processed multiple times in the same epoch, that is considered finished when all images from $\mathcal{U}$ are processed once. This is done to avoid data imbalance, as the number of training frames from $\mathcal{S}$ decrease relatively to $\mathcal{U}$. 

Results obtained using this training schedule are shown in Table \ref{tab:ablation}, indicating that our proposed method statistically did not degrade when observing only $10000$ images, roughly $25\%$ of the total of annotated depth maps. Additionally, when observing only $1000$ images, or $2.5\%$ the total number of annotated depth maps, our proposed methods achieved performance comparable to \citet{SemiLeftRight} and \citet{luo2018single}, considered the current state-of-the-art for semi-supervised monocular depth estimation. As we further decrease the number of supervised frames, performance starts to degrade more steeply, however these are mostly due to the model's inability to learn proper scale with such sparse (and possibly biased) information. %This is shown in Fig. \ref{fig:decrease_frame}, where we can see that the overall shape of depth maps is still preserved as less supervised information is available. %Interestingly, we also see significant degradation in the reconstruction of areas not observed by the LiDAR sensor. As discussed in the previous section, this could be attributed to the ratio between the self-supervised and supervised losses during the training, that if not properly selected leads to such behavior. While we have used weights that are optimal for semi-supervision using all available depth maps, the imbalance generated by removing a certain amount could change the optimal values for these weights, requiring a more careful selection, however this is not explored here and is left for future work. 

\input{sections/06supmat_decrease_frame_table.tex}


\section{Effects of Beam Selection for Sparse Depth Labels}

In this section we explore how sensitive our semi-supervised depth estimates are to the selection of beams at training time, particularly as depth labels become sparser. In other words, we would like to investigate how the distribution of valid depth pixels throughout annotated labels impact overall results. In our original experiments, beam sparsification was achieved by keeping only those at equally spaced intervals, and by increasing these intervals the number of beams decreases. Naturally, when all 64 beams are used there is no interval, when 32 are used every second beam is kept, when 16 are used every fourth beam is kept, and so forth. It is important to note that not all beams are necessarily used by the reprojected depth map, since their point of contact might not be visible by the camera. In fact, we noticed that most of the information contained in beams below the 45$^{th}$ is discarded, which makes the task of sparse semi-supervision even more challenging.

\input{sections/06supmat_beam_selection.tex}

In order to vary the position of depth information in the resulting sparse labels, while maintaining a proper distribution similar to what a real LiDAR sensor would provide, we opted for introducing an offset, determining where the top beam is located. Starting from 0, this offset increases until it coincides with another beam that was selected when no offset is considered. Following this strategy, when 32 beams are considered there are 2 variations, when 16 beams are considered there are 4, and so forth. The results when using this strategy are depicted in Fig. \ref{fig:beamsoffset}, where we can see that sparser depth labels are more sensitive to the distribution of valid pixels, and there are indeed some configurations that lead to better results, however there was no configuration that resulted in catastrophic failures. Interestingly, as we further increased sparsity, considering only 2 or even 1 beam, some configurations failed to converge, showing that there is a limit to how much sparsity  can be properly leveraged in our proposed semi-supervised learning framework, however a more thorough analysis is left for future work.

\input{sections/06supmat_videoframes.tex}

\section{Additional Qualitative Results}
Here we provide some more qualitative results of our proposed semi-supervised monocular depth estimation methodology, using the reprojected distance loss, on the KITTI dataset. Fig. \ref{fig:supqualitative} shows corresponding input RGB images and output depth maps, while Fig. \ref{fig:videobeams} depicts reconstructed pointclouds from models trained using different numbers of LiDAR beams. More qualitative results can be found on the supplementary video attached.


\input{sections/06supmat_qualitative.tex}



